Conflict-driven Inductive Logic Programming

The goal of Inductive Logic Programming (ILP) is to learn a program that explains a set of examples. Until recently, most research on ILP targeted learning Prolog programs. The ILASP system instead learns Answer Set Programs (ASP). Learning such expressive programs widens the applicability of ILP considerably; for example, enabling preference learning, learning common-sense knowledge, including defaults and exceptions, and learning non-deterministic theories. Early versions of ILASP can be considered meta-level ILP approaches, which encode a learning task as a logic program and delegate the search to an ASP solver. More recently, ILASP has shifted towards a new method, inspired by conflict-driven SAT and ASP solvers. The fundamental idea of the approach, called Conflict-driven ILP (CDILP), is to iteratively interleave the search for a hypothesis with the generation of constraints which explain why the current hypothesis does not cover a particular example. These coverage constraints allow ILASP to rule out not just the current hypothesis, but an entire class of hypotheses that do not satisfy the coverage constraint. This paper formalises the CDILP approach and presents the ILASP3 and ILASP4 systems for CDILP, which are demonstrated to be more scalable than previous ILASP systems, particularly in the presence of noise. Under consideration in Theory and Practice of Logic Programming (TPLP).

==> conflict_analysis/ilasp3_cdpi.tex <==

%\subsubsection{Translating a CDPI}
\label{sec:cdpi_translation}

When translating a CDPI $e$, the coverage formula computed by ILASP3 is a
disjunction $D_1\lor \ldots\lor D_n$, which is constructed iteratively. The
intuition is that in the $i^{th}$ iteration the algorithm searches for a
hypothesis that accepts $e$, but which is not accepted by
$D_1\lor\ldots\lor D_{i-1}$. To prove that the example is accepted by such a
hypothesis $H$ the algorithm tries to find an answer set of $B\cup e_{ctx}\cup
H$ that extends $e_{pi}$. If such an answer set $I$ exists, a coverage formula
$D_i$ is computed (and added to the disjunction) s.t.\ $D_i$ is accepted by
exactly those hypotheses $H'$ s.t.\ $I\in AS(B\cup e_{ctx}\cup H')$. If no such
answer set exists then $F = D_1\lor\ldots\lor D_{i-1}$ is necessary for the
example to be accepted. If the example $e$ is positive, then $\langle e,
F\rangle$ is a coverage constraint; if $e$ is negative then $\langle e, \lnot
F\rangle$ is a coverage constraint.

This incremental computation relies on being able to generate from an
interpretation $I$ a coverage formula that is accepted by exactly those
hypotheses $H$ such that $I\in AS(B \cup e_{ctx}\cup H)$. A general
formalisation of such a coverage formula is given in the following definition.
Note that the definition is strongly linked to the unfounded sets definition of
answer sets (given in the Section 2), which says that answer sets of a program
$P$ are the models of $P$ with no non-empty unfounded subsets.

\begin{definition}
  Let $I$ be an interpretation and $e$ be a CDPI. The \emph{translation} of
  $\langle I, e\rangle$ (denoted $\mathcal{T}(I, e, T)$) is the coverage
  formula constructed by taking the conjunction of the following coverage
  formulas:

  \begin{enumerate}
    \item $\lnot R_{id}$ for each $R \in S_M$ such that $I$ is not a model of
      $R$.
    \item $R_{id}^1\lor\ldots\lor R_{id}^n$ for each subset minimal set of
      rules $\lbrace R^1,\ldots,R^n\rbrace$ such that there is at least one
      non-empty unfounded subset of $I$ \wrt $B\cup e_{ctx}\cup
      (S_{M}\backslash \lbrace R^1,\ldots,R^n\rbrace)$.
  \end{enumerate}

  We write $\mathcal{T}_1(I, e, T)$ and $\mathcal{T}_2(I, e, T)$ to refer to
  the conjunctions of coverage formulas in (1) and (2), respectively. Note that
  the empty conjunction is equal to $\top$.
\end{definition}

\begin{example}\label{eg:translate}
  Consider an $\loasne$ task with background knowledge $B$ and hypothesis space
  $S_M$ as defined below.

  \begin{multicols}{2}

    $B = \left\{\begin{array}{l}
      \asp{p \codeif \naf q.}\\
      \asp{q \codeif \naf p.}\\
    \end{array}\right\}$

    $S_M = \left\{ \begin{array}{rl}
        h^1:& \asp{r \codeif t.}\\
        h^2:& \asp{t \codeif q.}\\
        h^3:& \asp{r.}\\
      \end{array}
    \right\}$

  \end{multicols}

  Let $e$ be a CDPI such that $e_{pi} = \langle \lbrace \asp{r}\rbrace,
  \emptyset\rangle$, and $e_{ctx} = \emptyset$. Consider the three
  interpretations $I_1 = \lbrace \asp{p}$, $\asp{r}\rbrace$, $I_2 = \lbrace
  \asp{q}$, $\asp{r}\rbrace$ and $I_3 = \lbrace \asp{q}$, $\asp{r}$,
  $\asp{t}\rbrace$. The translations are as follows:

  \begin{itemize}
    \item $\mathcal{T}(I_1, e, T) = h^3_{id}$.
    \item $\mathcal{T}(I_2, e, T) = \lnot h^2_{id} \land h^3_{id}$.
    \item $\mathcal{T}(I_3, e, T) = h^2_{id} \land (h^1_{id} \lor h^3_{id})$.
  \end{itemize}
\end{example}

The following theorem shows that the translation of an interpretation $I$
(w.r.t.\ an example $e$) is a coverage formula that captures the class of
hypotheses $H$ for which $I$ is an accepting answer set of $B\cup H$ w.r.t.\
$e$.

\appendixTheoremHere{translateCDPI}{
  Let $e$ be a CDPI and $I$ be a model of $B\cup e_{ctx}$. For any hypothesis
  $H\subseteq S_{M}$, $I \in AS(B\cup H \cup e_{ctx})$ accepts $e$ if and only
  if the translation of $\langle I, e\rangle$ accepts $H$.
}{
  Assume $I \in AS(B\cup H \cup e_{ctx})$.

  \proofindent{
    $\Leftrightarrow I$ is a model of $B\cup H\cup e_{ctx}$ and there are no
    non-empty subsets of $I$ \wrt $B\cup H\cup e_{ctx}$

    $\Leftrightarrow I$ is a model of $H$ and there are no non-empty subsets of
    $I$ \wrt $B\cup H\cup e_{ctx}$ (as $I$ is a model of $B\cup e_{ctx}$)

    $\Leftrightarrow I$ is a model of $H$ and for each set of rules $\lbrace
    R^1,\ldots,R^n\rbrace$ s.t.\ there is a non-empty unfounded subset of $I$
    \wrt $B\cup e_{ctx}\cup (S_{M}\backslash \lbrace R^1,\ldots,R^n\rbrace)$,
    $H\cap \lbrace R^1,\ldots,R^n\rbrace \neq \emptyset$.

    $\Leftrightarrow I$ is a model of $H$ and for each subset minimal set of
    rules $\lbrace R^1,\ldots,R^n\rbrace$ s.t.\ there is a non-empty unfounded
    subset of $I$ \wrt $B\cup e_{ctx}\cup (S_{M}\backslash \lbrace
    R^1,\ldots,R^n\rbrace)$, $H\cap \lbrace R^1,\ldots,R^n\rbrace \neq
    \emptyset$.

    $\Leftrightarrow$ the translation of $\langle I, e\rangle$ accepts $H$.
  }
}

Algorithm~\ref{alg:translateEG} formalises the $\textit{translateCDPI}$
procedure used by ILASP3 to translate a CDPI into a coverage formula. It takes
an iterative approach, translating one interpretation per iteration until the
coverage formula $F$ becomes necessary for $e$ to be accepted.

\begin{algorithm}
  \begin{algorithmic}[1]
    \Procedure{translateCDPI}{$T, e$}
      \State{$F = \bot$;}
      \While{$\exists I$, $\exists H \subseteq S_M$ s.t.\ $F$ does not accept $H$ and $I\in AAS(e, B\cup H)$}
        \State{Fix an arbitrary such $I$}
        \State{$F = F \lor \mathcal{T}(I, e, T)$;}
      \EndWhile
      \State{\textbf{return}\,$F$;}
    \EndProcedure
  \end{algorithmic}
  \caption{$\textit{translateCDPI}(T, e)$ \label{alg:translateEG}}
\end{algorithm}

\begin{example}\label{eg:translateEG}
  Reconsider the $\loasne$ task from Example~\ref{eg:translate}. Let $e$ be the
  CDPI $\langle\langle \lbrace \asp{r}\rbrace, \emptyset\rangle,
  \emptyset\rangle$. The $\textit{translateCDPI}(T, e)$ procedure starts by
  initialising $F$ as $\bot$. In the first iteration, one interpretation $I$
  that satisfies the condition of the while loop is $\lbrace \asp{p,
  r}\rbrace$, with $H = \lbrace h^3\rbrace$. If this $I$ is selected in the
  first iteration then $F$ becomes $h^3_{id}$. In the second iteration, one
  possible interpretation that satisfies the condition of the while loop is
  $I=\lbrace \asp{p}$, $\asp{q}$, $\asp{r}\rbrace$, with $H = \lbrace h^1,
  h^2\rbrace$. If this $I$ is selected, then $F$ becomes $h^3_{id}\lor
  (h^2_{id} \land (h^1_{id}\lor h^3_{id}))$. There are no further $I$'s that
  can satisfy the condition of the while loop, so $F$ is returned.
\end{example}

Example~\ref{eg:translateEG} demonstrates that it is not always necessary to
translate every interpretation that could be an accepting answer set of $e$. In
fact, it is often possible to translate a much smaller set of interpretations.
Theorem~\ref{thm:translateEGterminate} proves that $\textit{translateCDPI}$  is
guaranteed to terminate, and Theorem~\ref{thm:translateEG} proves that the
returned coverage formula (negated in the case of a negative example) can be
used as a coverage constraint for $e$. As the theorem shows that there is no
hypothesis that is accepted by the coverage formula that does not cover $e$,
when the algorithm is used as a method for conflict analysis on the most recent
hypothesis $H$ (which does not cover $e$), the coverage formula must not accept
$H$. Hence, the approach in this section is a valid method for conflict
analysis.

\appendixTheorem{translateEGterminate}{
  Let $e$ be a CDPI. The procedure $\textit{translateCDPI}(T, e)$ is guaranteed
  to terminate.
}{
  It suffices to show that there is a finite number of iterations of the while
  loop, which must be the case if the number of hypotheses $H\subseteq S_M$
  accepted by $F$ increases with every iteration (as $S_{M}$ is finite). As
  each new iteration only adds an extra disjunct to $F$, it is clear that the
  hypotheses accepted by $F$ cannot decrease; hence, it remains to show that at
  least one new hypothesis is accepted by $F$ in each iteration. For the
  condition of the while loop to hold, at the start of an arbitrary iteration
  there must be a hypothesis $H \subseteq S_M$ which is not accepted by $F$ and
  for which there is at least one $I\in AAS(e, B\cup H)$. For any such $I$, $H$
  must be accepted by $\mathcal{T}(I, e, T)$ (by
  Theorem~\ref{thm:translateCDPI}), and thus $F$ at the end of the iteration;
  thus $H$ is a formula that is not accepted by $F$ at the start of the
  iteration, but is accepted by $F$ at the end of the iteration.
}

\appendixTheorem{translateEG}{
  Let $e$ be a CDPI and let $F$ be the coverage formula returned by
  $\textit{translateCDPI}(T, e)$.
  \begin{enumerate}
    \item If $e\in E^{+}$, the pair $\langle e, F\rangle$ is a coverage
      constraint and there is no hypothesis accepted by $F$ that covers $e$.
    \item If $e\in E^{-}$, the pair $\langle e, \lnot F\rangle$ is a coverage
      constraint and there is no hypothesis accepted by $\lnot F$ that covers
      $e$.
  \end{enumerate}
}{
  To prove both parts of the theorem it suffices to show that for any
  $H\subseteq S_{M}$, $F$ is accepted $H$ if and only if there is at least one
  accepting answer set of $e$ \wrt $B\cup H$.

  \noindent
  \textit{Proof of $\Rightarrow$}. Assume that $F$ accepts $H$. Then $H$ is
  accepted by at least one of the disjuncts in $F$. Then there must be at least
  one interpretation $I$ that is an accepting answer set of $e$ \wrt $B\cup H'$
  (for at least one $H'$) s.t.\ $H$ is accepted by $\mathcal{T}(I, e, T)$. As $I$
  is an accepting answer set, it must extend $e_{pi}$. Hence, by
  Theorem~\ref{thm:translateCDPI}, $I$ is an accepting answer set of $e$ \wrt
  $B\cup H$.

  \noindent
  \textit{Proof of $\Leftarrow$}. Let $I$ be an accepting answer set of $e$
  \wrt $B\cup H$ and assume for contradiction that $F$ does not accept $H$.
  Then the while loop in $\textit{translateCDPI}(T, e)$ could not have
  terminated. This contradiction shows that $F$ must accept $H$.
}


==> conflict_analysis/ilasp4_cdoe_brave.tex <==
\subsubsection*{Necessary Constraints for Brave Ordering Examples}

Similarly to the approach taken for positive and negative CDPIs in the main
paper, ILASP4 computes a coverage formula which is necessary but not sufficient
to cover brave and cautious CDOE examples. This section formalises the approach
for brave orderings and the next section formalises the approach for cautious
orderings. The algorithm in this section is similar to the CDPI2NC approach in
the main paper, but adapted for brave orderings. Again, in each iteration only
a single condition from the full translation of the ordering example is
selected. Just as is the case for the CDPI2NC algorithm, the CDOE2NC algorithm
(Algorithm~\ref{alg:CDOE2NC1}) is guaranteed to produce a coverage formula
which does not accept the most recent hypothesis but is necessary for the brave
ordering example to be covered.

\begin{algorithm}
  \begin{algorithmic}[1]
    \Procedure{CDOE2NC}{$T, H, e_1, e_2, \prec$}
      \State{$F = \bot$;}
      \While{$\exists \langle I_1, I_2\rangle$ s.t.\ $\exists H'\subseteq S_M$ st
             $F$ does not accept $H'$, $I_1 \in \textit{AAS}(e_1, B\cup
             H)$, $I_1 \in \textit{AAS}(e_1, B\cup H')$, $I_2
             \in \textit{AAS}(e_2, B\cup H)$, $I_2
             \in \textit{AAS}(e_2, B\cup H')$ and $I_1 \prec_{B\cup H'} I_2$}
        \State{Fix an arbitrary such $\langle I_1, I_2\rangle$}
        \State{$F = F \lor \omega(T, I_1, I_2, \prec)$;}
      \EndWhile
      \While{$\exists \langle I_1, I_2\rangle$ s.t.\ $\exists H'\subseteq S_M$ st
             $F$ does not accept $H'$, $I_1 \in \textit{AAS}(e_1, B\cup H')$, $I_2
             \in \textit{AAS}(e_2, B\cup H')$, $I_1, I_2\in M(H)$ and $I_1 \prec_{B\cup H'} I_2$}
        \State{Fix an arbitrary such $\langle I_1, I_2\rangle$}
        \State{Let $d$ be an arbitrary conjunct of $\mathcal{T}_2(I_1, e_1, T)$
        or $\mathcal{T}_2(I_2, e_2, T)$ that does not accept $H$;}
        \State{$F = F \lor d$;}
      \EndWhile
      \While{$\exists \langle I_1, I_2\rangle$ s.t.\ $\exists H'\subseteq S_M$ st
             $F$ does not accept $H'$, $I_1 \in \textit{AAS}(e_1, B\cup H')$, $I_2
             \in \textit{AAS}(e_2, B\cup H')$ and $I_1 \prec_{B\cup H'} I_2$}
        \State{Fix an arbitrary such $\langle I_1, I_2\rangle$}
        \State{$F = F \lor (\mathcal{T}_1(I_1, e_1, T)\land \mathcal{T}_1(I_2, e_2, T))$;}
      \EndWhile
      \State{\textbf{return}\,$F$;}
    \EndProcedure
  \end{algorithmic}
  \caption{$\textit{CDOE2NC}(T, H, e_1, e_2, \prec)$ \label{alg:CDOE2NC1}}
\end{algorithm}

The following two theorems demonstrate that the CDOE2NC algorithm is guaranteed
to terminate and can be used as part of a valid method for conflict analysis on
brave ordering examples.

\appendixTheorem{cdoe_to_nc1_terminate}{
  Let $o = \langle e_1, e_2, \prec\rangle$ be a CDOE in $O^{b}$ and $H\subseteq
  S_{M}$ be a hypothesis that does not cover $o$. The procedure
  $\textit{CDOE2NC}(T, H, e_1, e_2, \prec)$ is guaranteed to terminate.
}{
  (Similar to the proof of Theorem~\ref{thm:cdpi_to_nc1_terminate}).

  As $F$ is a disjunction, and each iteration of all three while loops adds an
  extra disjunct, the hypotheses $H\subseteq S_M$ accepted must either increase
  or stay the same with each iteration (of each while loop). Hence as there are
  a finite number of hypotheses (because $S_M$ is finite), it remains to show
  that for each of the three while loops each iteration adds at least one
  hypothesis that is accepted by $F$ at the end of the iteration that was not
  accepted by $F$ at the start of the iteration.

  In any iteration of the first while loop, there is at least one $H'\subseteq
  S_M$ s.t.\ $H'$ is not accepted by $F$ and $\exists \langle I_1, I_2\rangle$
  s.t.\ $I_1 \in \textit{AAS}(e_1, B\cup H)$, $I_1 \in \textit{AAS}(e_1, B\cup
  H')$, $I_2 \in \textit{AAS}(e_2, B\cup H)$, $I_2 \in \textit{AAS}(e_2, B\cup
  H')$ and $I_1 \prec_{B\cup H'} I_2$. It therefore suffices to show that $H'$
  is accepted by the new disjunct $d = \omega(T, I_1, I_2, \prec)$. This
  follows from Theorem~\ref{thm:omega}.

  In any iteration of the second while loop there is at least one $H' \subseteq
  S_M$ st $H'$ is not accepted by $F$, $I_1 \in \textit{AAS}(e_1, B\cup H')$,
  $I_2 \in \textit{AAS}(e_2, B\cup H')$, $I_1, I_2\in M(H)$ and $I_1
  \prec_{B\cup H'} I_2$ (where $\langle I_1, I_2\rangle$ is the arbitrarily
  chosen $\langle I_1, I_2\rangle$). Note that the arbitrary selection of $d$
  is well defined as at least one of $\mathcal{T}_2(I_1, e_1, T)$ and
  $\mathcal{T}_2(I_2, e_2, T)$ must have at least one conjunct that does not
  accept $H$ -- otherwise neither $I_1$ nor $I_2$ could have any non-empty
  unfounded subsets \wrt $B\cup (e_1)_{ctx}\cup H$ and $B\cup (e_2)_{ctx}\cup
  H$ (respectively), and as $I_1$ and $I_2$ are models of $B\cup
  (e_1)_{ctx}\cup H$ and $B\cup (e_2)_{ctx}\cup H$ (respectively) and $I_1
  \prec_{B\cup H'} I_2$, this would contradict the fact that the first while
  loop terminated. Without loss of generality, assume that $d$ is from
  $\mathcal{T}_2(I_1, e_1, T)$. It suffices to show that $H'$ is accepted by
  the new disjunct $d$, which is of the form $R^1_{id}\lor\ldots\lor
  R^{n}_{id}$, where $I_1$ has at least one non-empty unfounded subset \wrt
  $B\cup e_{ctx}\cup (S_{M}\backslash \lbrace R^{1},\ldots, R^{n}\rbrace)$. If
  $H'$ were not accepted by $d$, then $B\cup e_{ctx} \cup H'$ would be a subset
  of $B\cup e_{ctx} \cup (S_{M}\backslash \lbrace R^{1},\ldots, R^{n}\rbrace)$,
  and $I_1$ would therefore have at least one non-empty unfounded subset \wrt
  the program, contradicting that $I_1\in AAS(e_1, B\cup H')$.

  In any iteration of the third while loop, there must be at least one $H'
  \subseteq S_M$ st $H'$ is not accepted by $F$, $I_1 \in \textit{AAS}(e_1,
  B\cup H')$, $I_2 \in \textit{AAS}(e_2, B\cup H')$ and $I_1 \prec_{B\cup H'}
  I_2$ (where $\langle I_1, I_2\rangle$ is the arbitrarily chosen $\langle I_1,
  I_2\rangle$). As the second while loop terminated, $I_1$ and $I_2$ cannot
  both be models of $H$. Hence, $\mathcal{T}_1(I_1, e_1, T)
  \land\mathcal{T}_1(I_2, e_2, T)$ must be a non-empty conjunction $\lnot
  R^{1}_{id}\land\ldots\land \lnot R^{n}_{id}$ of rules s.t.\ for each each
  $R^{i}$ at least one of $I_1$ or $I_2$ is not a model (it must be non-empty
  because there is at least one rule in $H$, and therefore in $S_{M}$, for
  which either $I_1$ or $I_2$ is not a model). As $I_1$ (resp.  $I_2$) is a
  model of $B\cup (e_1)_{ctx}\cup H'$ (resp. $B\cup (e_2)_{ctx}\cup H'$), $H'$
  cannot contain any of the rules whose ids are in $\mathcal{T}_1(I_1, e_1,
  T)\land \mathcal{T}_1(I_2, e_2, T)$; hence $H'$ is a hypothesis that is not
  accepted by $F$ at the start of the iteration, but which is accepted by $F$
  at the end of the iteration.
}

\appendixTheorem{cdoe_to_nc1}{
  Let $o = \langle e_1, e_2, \prec\rangle$ be a CDOE in $O^{b}$ and
  $H\subseteq S_{M}$ be a hypothesis that does not cover $o$. Let $F$ be the
  coverage formula returned by $\textit{CDOE2NC}(T, H, e_1, e_2, \prec)$.
  \begin{enumerate}
    \item $F$ does not accept $H$.
    \item The pair $\langle o, F\rangle$ is a coverage constraint.
  \end{enumerate}
}{
  \proofindent{
    \begin{enumerate}
      \item To prove this part, it suffices to show that $H$ cannot accept the
        disjunct that is added in an arbitrary iteration of any of the three
        while loops. For the first while loop, by Theorems~\ref{thm:omega}, if
        $H$ is accepted by the new disjunct then $I_1\prec_{B\cup H} I_2$.
        Hence, as $I_1\in \textit{AAS}(e_1, B\cup H)$ and $I_2\in
        \textit{AAS}(e_2, B\cup H)$, this cannot be the case (because $H$ does
        not cover $o$).  For the second while loop, this holds by definition.
        For the third while loop, this holds because the new disjunct is a
        conjunction $\lnot R^{1}_{id}\land\ldots\land \lnot R^{n}_{id}$ where
        at least one $R^{i}$ is in $H$ (if this were not the case then $I_1$
        and $I_2$ would both be models of $H$, which cannot be the case because
        the second while loop terminated).
      \item When $F$ is returned, the condition of the third while loop must be
        false; hence, there is no $\langle I_1, I_2\rangle$ for which $\exists
        H'\subseteq S_M$ s.t.\ $F$ does not accept $H$, $I_1 \in
        \textit{AAS}(e_1, B\cup H')$, $I_2 \in \textit{AAS}(e_2, B\cup H')$ and
        $I_1 \prec_{B\cup H'} I_2$ -- this is the definition of $\langle o,
        F\rangle$ being a coverage constraint.
    \end{enumerate}
  }
}


==> conflict_analysis/ilasp4_cdoe_brave_extended.tex <==
\subsubsection*{A middle ground approach for brave orderings}

Similarly to the approach taken in the main paper for positive CDPIs, there is
also a ``middle ground'' approach for brave ordering examples. Just as in the
CDPI2NCb method, the changes made to the CDOE2NC method to generate the
CDOE2NCb are very small and only involve changing one of the while loops (in
this case, the second while loop). The ILASP4b method used in the evaluation
uses this CDOE2NCb method rather than the CDOE2NC method.

\begin{algorithm}
  \begin{algorithmic}[1]
    \Procedure{CDOE2NCb}{$T, H, e_1, e_2, \prec$}
      \State{$F = \bot$;}
      \While{$\exists \langle I_1, I_2\rangle$ s.t.\ $\exists H'\subseteq S_M$ st
             $F$ does not accept $H'$, $I_1 \in \textit{AAS}(e_1, B\cup
             H)$, $I_1 \in \textit{AAS}(e_1, B\cup H')$, $I_2
             \in \textit{AAS}(e_2, B\cup H)$, $I_2
             \in \textit{AAS}(e_2, B\cup H')$ and $I_1 \prec_{B\cup H'} I_2$}
        \State{Fix an arbitrary such $\langle I_1, I_2\rangle$}
        \State{$F = F \lor \omega(T, I_1, I_2, \prec)$;}
      \EndWhile
      \While{$\exists \langle I_1, I_2\rangle$ s.t.\ $\exists H'\subseteq S_M$ st
             $F$ does not accept $H'$, $I_1 \in \textit{AAS}(e_1, B\cup H')$, $I_2
             \in \textit{AAS}(e_2, B\cup H')$, $I_1, I_2\in M(H)$ and $I_1 \prec_{B\cup H'} I_2$}
        \State{Fix an arbitrary such $\langle I_1, I_2\rangle$}
        \State{$F = F \lor (\mathcal{T}_2(I_1, e_1, T)\land \mathcal{T}_2(I_2, e_2, T))$;}
      \EndWhile
      \While{$\exists \langle I_1, I_2\rangle$ s.t.\ $\exists H'\subseteq S_M$ st
             $F$ does not accept $H'$, $I_1 \in \textit{AAS}(e_1, B\cup H')$, $I_2
             \in \textit{AAS}(e_2, B\cup H')$ and $I_1 \prec_{B\cup H'} I_2$}
        \State{Fix an arbitrary such $\langle I_1, I_2\rangle$}
        \State{$F = F \lor (\mathcal{T}_1(I_1, e_1, T)\land \mathcal{T}_1(I_2, e_2, T))$;}
      \EndWhile
      \State{\textbf{return}\,$F$;}
    \EndProcedure
  \end{algorithmic}
  \caption{$\textit{CDOE2NCb}(T, H, e_1, e_2, \prec)$ -- extract \label{alg:CDOE2NCb}}
\end{algorithm}

The following two theorems demonstrate that the CDOE2NCb algorithm is guaranteed
to terminate and can be used as part of a valid method for conflict analysis on
brave ordering examples.

\appendixTheorem{cdoe_to_nc2_terminate}{
  Let $o = \langle e_1, e_2, o_{op}\rangle$ be a CDOE in $O^{b}$ and
  $H\subseteq S_{M}$ be a hypothesis that does not cover $o$. The procedure
  $\textit{CDOE2NCb}(T, H, e_1, e_2, \prec)$ is guaranteed to terminate.
}{
  (Similar to the proof of Theorem~\ref{thm:cdoe_to_nc1_terminate}).

  As $F$ is a disjunction, and each iteration of all three while loops adds an extra
  disjunct, the hypotheses $H\subseteq S_M$ accepted must either increase or
  stay the same with each iteration (of each while loop). Hence as there are
  a finite number of hypotheses (because $S_M$ is finite), it remains to show
  that for each of the three while loops each iteration adds at least one
  hypothesis that is accepted by $F$ at the end of the iteration that was not
  accepted by $F$ at the start of the iteration.

  In any iteration of the first while loop, there is at least one $H'\subseteq
  S_M$ s.t.\ $H'$ is not accepted by $F$ and $\exists \langle I_1, I_2\rangle$
  s.t.\ $I_1 \in \textit{AAS}(e_1, B\cup H)$, $I_1 \in \textit{AAS}(e_1, B\cup
  H')$, $I_2 \in \textit{AAS}(e_2, B\cup H)$, $I_2 \in \textit{AAS}(e_2, B\cup
  H')$ and $I_1 \prec_{B\cup H'} I_2$. It therefore suffices to show that $H'$
  is accepted by the new disjunct $d = (\mathcal{T}(I_1, e, T)\land
  \mathcal{T}(I_2, e, T) \land \omega(T, I_1, I_2, \prec)$. This follows from
  Theorems~\ref{thm:translateCDPI} and~\ref{thm:omega}.

  In any iteration of the second while loop there is at least one $H' \subseteq
  S_M$ st $H'$ is not accepted by $F$, $I_1 \in \textit{AAS}(e_1, B\cup H')$,
  $I_2 \in \textit{AAS}(e_2, B\cup H')$, $I_1, I_2\in M(H)$ and $I_1
  \prec_{B\cup H'} I_2$ (where $\langle I_1, I_2\rangle$ is the arbitrarily
  chosen $\langle I_1, I_2\rangle$). It suffices to show that $H'$ is accepted
  by the new disjunct $\mathcal{T}_2(I_1, e_1, T)\land\mathcal{T}_2(I_2, e_2,
  T)$, which is a conjunction of disjunctions; hence, we must show that $H'$ is
  accepted by each of these disjunctions. Each disjunction is of the form
  $R^1_{id}\lor\ldots\lor R^{n}_{id}$, where $I_1$ (w.l.o.g.) has at
  least one non-empty unfounded subset \wrt $B\cup (e_1)_{ctx}\cup
  (S_{M}\backslash \lbrace R^{1},\ldots, R^{n}\rbrace)$. If $H'$ were not
  accepted by $d$, then $B\cup e_{ctx} \cup H'$ would be a subset of $B\cup
  (e_1)_{ctx} \cup (S_{M}\backslash \lbrace R^{1},\ldots, R^{n}\rbrace)$, and
  $I_1$ would therefore have at least one non-empty unfounded subset \wrt the
  program, contradicting that $I_1\in AAS(e_1, B\cup H')$.

  In any iteration of the third while loop, there must be at least one $H'
  \subseteq S_M$ st $H'$ is not accepted by $F$, $I_1 \in \textit{AAS}(e_1,
  B\cup H')$, $I_2 \in \textit{AAS}(e_2, B\cup H')$ and $I_1 \prec_{B\cup H'}
  I_2$ (where $\langle I_1, I_2\rangle$ is the arbitrarily chosen $\langle I_1,
  I_2\rangle$). As the second while loop terminated, $I_1$ and $I_2$ cannot
  both be models of $H$. Hence, $\mathcal{T}_1(I_1, e_1, T)
  \land\mathcal{T}_1(I_2, e_2, T)$ must be a non-empty conjunction $\lnot
  R^{1}_{id}\land\ldots\land \lnot R^{n}_{id}$ of rules s.t.\ for each each
  $R^{i}$ at least one of $I_1$ or $I_2$ is not a model (it must be non-empty
  because there is at least one rule in $H$, and therefore in $S_{M}$, for
  which either $I_1$ or $I_2$ is not a model). As $I_1$ (resp.  $I_2$) is a
  model of $B\cup (e_1)_{ctx}\cup H'$ (resp. $B\cup (e_2)_{ctx}\cup H'$), $H'$
  cannot contain any of the rules whose ids are in $\mathcal{T}_1(I_1, e_1,
  T)\land \mathcal{T}_1(I_2, e_2, T)$; hence $H'$ is a hypothesis that is not
  accepted by $F$ at the start of the iteration, but which is accepted by $F$
  at the end of the iteration.
}

\appendixTheorem{cdoe_to_nc2}{
  Let $o = \langle e_1, e_2, o_{op}\rangle$ be a CDOE in $O^{b}$ and
  $H\subseteq S_{M}$ be a hypothesis that does not cover $o$. Let $F$ be the
  coverage formula returned by $\textit{CDOE2NCb}(T, H, e_1, e_2, \prec)$.
  \begin{enumerate}
    \item $F$ does not accept $H$.
    \item The pair $\langle o, F\rangle$ is a coverage constraint.
  \end{enumerate}
}{
  \proofindent{
    (Similar to the proof of Theorem~\ref{thm:cdoe_to_nc1}).
    \begin{enumerate}
      \item To prove this part, it suffices to show that $H$ cannot accept the
        disjunct that is added in an arbitrary iteration of any of the three
        while loops. For the first while loop, by Theorems~\ref{thm:omega}, if
        $H$ is accepted by the new disjunct then $I_1\prec_{B\cup H} I_2$.
        Hence, as $I_1\in \textit{AAS}(e_1, B\cup H)$ and $I_2\in
        \textit{AAS}(e_2, B\cup H)$, this cannot be the case (because $H$ does
        not cover $o$).

        For the second while loop, if $H$ were to be accepted by
        $\mathcal{T}_2(I_1, e_1, T) \land\mathcal{T}_2(I_2, e_2, T)$ then $H$
        would be accepted by both $\mathcal{T}(I_1, e_1, T)$ and
        $\mathcal{T}(I_2, e_2, T)$ (as $I_1$ and $I_2$ are models of $H$). By
        Theorem~\ref{thm:translateCDPI}, this would mean that $I_1 \in AAS(e_1,
        B\cup H)$ and $I_2 \in AAS(e_2, B\cup H)$, which cannot be the case or
        the first while loop would not have terminated. Hence, $H$ cannot be
        accepted by the new disjunct.

        For the third while loop, this holds because the new disjunct is a
        conjunction $\lnot R^{1}_{id}\land\ldots\land \lnot R^{n}_{id}$ where
        at least one $R^{i}$ is in $H$ (if this were not the case then $I_1$
        and $I_2$ would both be models of $H$, which cannot be the case because
        the second while loop terminated).
      \item When $F$ is returned, the condition of the third while loop must be
        false; hence, there is no $\langle I_1, I_2\rangle$ for which $\exists
        H'\subseteq S_M$ s.t.\ $F$ does not accept $H$, $I_1 \in
        \textit{AAS}(e_1, B\cup H')$, $I_2 \in \textit{AAS}(e_2, B\cup H')$ and
        $I_1 \prec_{B\cup H'} I_2$ -- this is the definition of $\langle e,
        F\rangle$ being a coverage constraint.
    \end{enumerate}
  }
}


==> conflict_analysis/ilasp4_cdoe_cautious.tex <==
\subsubsection*{Necessary Constraints for Cautious Ordering Examples}

Similarly to the ILASP4 approach to conflict analysis for negative examples, a
coverage constraint can be computed for a cautious ordering example by finding
a single pair of interpretations that are ordered incorrectly by the current
hypothesis. For a hypothesis to cover the ordering example, it must either not
accept one of the two interpretations as an answer set, or it must order them
correctly. The coverage formula expressing these three possibilities is
formalised and proven to be correct by the following theorem. The computation
of this formula is guaranteed to terminate, and the theorem shows that using
this formula is a valid method for conflict analysis on cautious ordering
examples.

\appendixTheorem{cdpi_to_c_ord_nc}{
  Let $o = \langle e_1, e_2, \prec\rangle$ be a CDOE in $O^{c}$ and
  $H\subseteq S_{M}$ be a hypothesis that does not cover $o$. There is at least
  one pair of interpretations $\langle I_1, I_2\rangle$ such that $I_1 \in
  \textit{AAS}(e_1, B\cup H)$, $I_2 \in \textit{AAS}(e_2, B\cup H)$ and
  $I_1 \prec^{-1}_{B\cup H} I_{2}$:
  \begin{enumerate}
    \item $\lnot \mathcal{T}(I_1, e_1, T)\lor \lnot\mathcal{T}(I_2, e_2, T)
      \lor \omega(T,I_1, I_2, \prec)$ does not accept $H$.
    \item $\langle o, \lnot \mathcal{T}(I_1, e_1, T)\lor \lnot\mathcal{T}(I_2,
      e_2, T) \lor \omega(T,I_1, I_2, \prec)\rangle$ is a coverage constraint.
  \end{enumerate}
}{
  As $H$ does not cover $o$, there must be at least one accepting pair of
  answer sets of $\langle e_1, e_2, \prec^{-1}\rangle$ \wrt $B\cup H$ (by definition
  of a cautious ordering example).
  \begin{enumerate}
    \item Let $\langle I_1, I_2\rangle$ be an arbitrary pair of interpretations
      $\langle I_1, I_2\rangle$ such that $I_1 \in \textit{AAS}(e_1, B\cup H)$,
      $I_2 \in \textit{AAS}(e_2, B\cup H)$ and $I_1 \prec^{-1}_{B\cup H}
      I_{2}$. By Theorem~\ref{thm:translateCDPI}, $\mathcal{T}(I_1, e_1, T)$
      and $\mathcal{T}(I_2, e_2, T)$ both accept $H$ and by
      Theorem~\ref{thm:omega} $\omega(T,I_1, I_2, \prec)$ does not accept $H$.
      Hence, $\lnot \mathcal{T}(I_1, e_1, T)\lor \lnot\mathcal{T}(I_2, e_2, T)
      \lor \omega(T,I_1, I_2, \prec)$ does not accept $H$.
    \item
      Let $H'$ be a hypothesis that covers $o$. It suffices to show that $H'$
      is accepted by $\lnot \mathcal{T}(I_1, e_1, T)\lor \lnot\mathcal{T}(I_2,
      e_2, T) \lor \omega(T,I_1, I_2, \prec)\rangle$. As $H'$ covers $o$,
      $\langle I_1, I_2\rangle$ cannot be an accepting pair of answer sets of
      $\langle e_1, e_2, \prec^{-1}\rangle$ \wrt $B\cup H'$. Hence, either $I_1
      \not\in \textit{AAS}(e_1, B\cup H)$, $I_2 \not\in \textit{AAS}(e_2, B\cup
      H)$ or $I_1 \prec_{B\cup H} I_{2}$; and hence, (by
      Theorems~\ref{thm:translateCDPI} and~\ref{thm:omega}) $H'$ is accepted by
      $\lnot \mathcal{T}(I_1, e_1, T)\lor \lnot\mathcal{T}(I_2,
      e_2, T) \lor \omega(T,I_1, I_2, \prec)\rangle$.
  \end{enumerate}
}


==> conflict_analysis/ilasp4_cdpi_negative.tex <==
\subsubsection{Necessary Constraints for Negative Examples}

The method for computing a necessary constraint for a negative CDPI $e$ is much
simpler than for positive CDPIs. Note that each disjunct in the formula $F$
computed by the translateCDPI method is sufficient but not necessary for the
CDPI $e$ to be accepted (i.e.\ for $e$ to not be covered, as it is a negative
example), and therefore its negation is necessary but not sufficient for $e$ to
be covered. This means that to compute a necessary constraint for a negative
CDPI, we only need to consider a single interpretation. This is formalised by
the following theorem. The approach used in ILASP4 computes an arbitrary such
coverage formula. Note that this is guaranteed to terminate and the following
theorem shows that the method is a valid method for conflict analysis.

\appendixTheorem{cdpi_to_neg_nc}{
  Let $e$ be a CDPI in $E^{-}$ and $H\subseteq S_{M}$ be a hypothesis that does
  not cover $e$. $\textit{AAS}(e, B\cup H)$ is non-empty and for any $I \in
  \textit{AAS}(e, B\cup H)$:
  \begin{enumerate}
    \item $\lnot \mathcal{T}(I, e, T)$ does not accept $H$.
    \item $\langle e, \lnot \mathcal{T}(I, e, T)\rangle$ is a coverage constraint.
  \end{enumerate}
}{
  As $H$ does not cover $e$, $\textit{AAS}(e, B\cup H)$ must be non-empty (by
  definition of a negative example).
  \begin{enumerate}
    \item Let $I$ be an arbitrary interpretation $I \in \textit{AAS}(e, B\cup
      H)$. By Theorem~\ref{thm:translateCDPI}, $\mathcal{T}(I, e, T)$ accepts
      $H$. Hence, $\lnot \mathcal{T}(I, e, T)$ does not accept $H$.
    \item
      Let $H'$ be a hypothesis that covers $e$. It suffices to show that $H'$
      is accepted by $\lnot \mathcal{T}(I, e, T)$. As $H'$ covers $e$, $I$
      cannot be an answer set of $B\cup e_{ctx} \cup H'$. Hence, by
      Theorem~\ref{thm:translateCDPI}, $\mathcal{T}(I, e, T)$ does not accept
      $H'$; hence $\lnot \mathcal{T}(I, e, T)$ accepts $H$.
  \end{enumerate}
}



==> conflict_analysis/ilasp4_cdpi_positive.tex <==
\subsubsection{Necessary Constraints for Positive Examples}

When the translation approach in the previous section is called, the CDILP
procedure has a current hypothesis $H$ and a counterexample CDPI $e$ that is
not covered. The translation approach ignores the current hypothesis $H$ and
computes a disjunction $F$ where each disjunct is a coverage formula which is
sufficient and necessary for a particular interpretation to be an answer set
(of $B\cup H\cup e_{ctx}$). As each disjunct is a conjunction of conditions
that are specific to that answer set, for the formula $F$ to be necessary to
accept $e$, $F$ is may contain a large number of disjuncts. In fact, if in each
iteration we were to pick only a single condition from the conjunction as the
disjunct, we would still end up with a necessary condition for $e$ to be
covered (any formula constructed in this way is guaranteed to be a consequence
of $F$), and is likely to contain fewer disjuncts and therefore be computed
faster; however, in general such a method is not valid -- as explained in
Section~\ref{sec:cdilp}, a valid method must always produce a coverage formula
which does not accept the most recent hypothesis (i.e.\ it should explain why
$e$ is a counterexample to $H$). In order to guarantee that the method is
valid, the approach in this section uses the most recent hypothesis to select
the condition for each disjunct. As each disjunct is sufficient for $e$ to be
covered at least one of its conjuncts must not be satisfied by $H$ (or $H$
would cover the example $e$). By selecting exactly one such conjunct from each
disjunct (rather than the full formula as in ILASP3), $F$ then becomes a much
smaller formula, which is essentially an explanation of why $H$ does not cover
$e$.

The approach is formalised by Algorithm~\ref{alg:CDPI2NC}. Note that in
general the approach could lead to many different coverage formulas, depending
on which conjunct is selected in each iteration. The approach in
Algorithm~\ref{alg:CDPI2NC} favours first selecting conditions from those
interpretations $I$ which can become answer sets if rules are added to $H$, and
then only when no such interpretations exist, selecting interpretations which
can become answer sets by removing rules from $H$. This is because it is more
costly to add rules (as it increases the hypothesis length) than to take them
away, so coverage formulas which are constructed in this way are likely to
``move the search on'' faster and lead to fewer iterations of the CDILP
procedure. However, this is only supported by intuition and initial
experimentation, and there may well be other selection strategies which perform
better -- future versions of ILASP will likely include many such selection
strategies.

\begin{algorithm}
  \small
  \begin{algorithmic}[1]
    \Procedure{CDPI2NC}{$T, H, e$}
      \State{$F = \bot$;}
      \While{$\exists I\!\in\! M(H)$, $\exists H'\!\subseteq\!S_M$ s.t.\ $F$ does not accept $H'$ and $I\!\in\!AAS(e, B\cup H')$}
        \State{Fix an arbitrary such $I$;}
        \State{Let $d$ be an arbitrary conjunct of $\mathcal{T}_2(I, e, T)$ that does not accept $H$;}
        \State{$F = F \lor d$;}
      \EndWhile
      \While{$\exists I$, $\exists H' \subseteq S_M$ s.t.\ $F$ does not accept $H'$ and $I\in AAS(e, B\cup H')$}
        \State{Fix an arbitrary such $I$;}
        \State{$F = F \lor \mathcal{T}_1(I, e, T)$;}
      \EndWhile
      \State{\textbf{return}\,$F$;}
    \EndProcedure
  \end{algorithmic}
  \caption{$\textit{CDPI2NC}(T, e)$ \label{alg:CDPI2NC}}
\end{algorithm}

\begin{example}\label{eg:compute_necessary_from_CDPI}
  Consider an $\loasne$ task with background knowledge $B$ and hypothesis space
  $S_M$ as defined below.

  \begin{multicols}{2}

    $B = \left\{\begin{array}{l}
      \asp{p \codeif \naf q.}\\
      \asp{q \codeif \naf p.}\\
      \asp{t \codeif s.}\\
    \end{array}\right\}$

    $S_M = \left\{ \begin{array}{rl}
        h^1:& \asp{t \codeif p.}\\
        h^2:& \asp{t \codeif q.}\\
        h^3:& \asp{r.}\\
        h^4:& \asp{s.}\\
      \end{array}
    \right\}$

  \end{multicols}

  Let $e$ be a CDPI such that $e_{pi} = \langle \lbrace \asp{t},
  \asp{r}\rbrace, \emptyset\rangle$, and $e_{ctx} = \emptyset$. And let $H =
  \lbrace h^3\rbrace$. If the translation approach of ILASP3 were to be used,
  the coverage formula $(\lnot h^4_{id} \land h^3_{id} \land (h^1_{id} \lor
  h^2_{id})) \lor (h^3_{id} \land h^4_{id})$ would be returned. The CDPI2NC
  approach instead returns $h^1_{id}\lor h^2_{id}\lor h^4_{id}$. Note that this
  formula is a consequence of the formula computed by the translation approach,
  and is therefore necessary for $e$ to be covered; however, it is not
  sufficient, meaning that in a future iteration, the hypothesis $H' = \lbrace
  h^1\rbrace$ may be learned, leading to $e$ again being a counterexample and
  the additional coverage formula $h^3_{id}$ being computed.
\end{example}

The following two theorems show that the CDPI2NC algorithm is guaranteed to
terminate and is a valid method for computing a coverage constraint for a
positive CDPI.

\appendixTheorem{cdpi_to_nc1_terminate}{
  Let $e$ be a CDPI in $E^{+}$ and $H\subseteq S_{M}$ be a hypothesis that does
  not cover $e$. The procedure $\textit{CDPI2NC}(T, H, e)$ is guaranteed to
  terminate.
}{
  As $F$ is a disjunction, and each iteration of both while loops adds an extra
  disjunct, the hypotheses $H\subseteq S_M$ accepted must either increase or
  stay the same with each iteration (of either while loop). Hence as there are
  a finite number of hypotheses (because $S_M$ is finite), it remains to show
  that for both while loops each iteration adds at least one hypothesis that is
  accepted by $F$ at the end of the iteration that was not accepted by $F$ at
  the start of the iteration.

  In any iteration of the first while loop there is at least one $H' \subseteq
  S_M$ st $H'$ is not accepted by $F$ and $I\in AAS(e, B\cup H')$ (where $I$ is
  the arbitrarily chosen $I$). Note that the arbitrary selection of $d$ is well
  defined as $\mathcal{T}_2(I, e, T)$ must have at least one conjunct that does
  not accept $H$ -- otherwise $I$ could not have any non-empty unfounded
  subsets \wrt $B\cup e_{ctx}\cup H$, and as $I$ is a model of $B\cup
  e_{ctx}\cup H$, this would contradict the fact that $H$ does not cover $e$.
  It therefore suffices to show that $H'$ is accepted by the new disjunct $d$,
  which is of the form $R^1_{id}\lor\ldots\lor R^{n}_{id}$, where $I$ has at
  least one non-empty unfounded subset \wrt $B\cup e_{ctx}\cup (S_{M}\backslash
  \lbrace R^{1},\ldots, R^{n}\rbrace)$. If $H'$ were not accepted by $d$, then
  $B\cup e_{ctx} \cup H'$ would be a subset of $B\cup e_{ctx} \cup
  (S_{M}\backslash \lbrace R^{1},\ldots, R^{n}\rbrace)$, and $I$ would
  therefore have at least one non-empty unfounded subset \wrt the program,
  contradicting that $I\in AAS(e, B\cup H')$.

  In any iteration of the second while loop, there must be at least one $H'
  \subseteq S_M$ st $H'$ is not accepted by $F$ and $I\in AAS(e, B\cup H')$.
  $I$ cannot be a model of $H$, or the first while loop would not have
  terminated. Hence, $\mathcal{T}_1(I, e, T)$ must be a non-empty conjunction
  $\lnot R^{1}_{id}\land\ldots\land \lnot R^{n}_{id}$ of rules s.t. $I$ is not
  a model of each $R^{i}$ (it must be non-empty because there is at least one
  rule in $H$, and therefore in $S_{M}$, for which $I$ is not a model). As $I$
  is a model of $B\cup e_{ctx}\cup H'$, $H'$ cannot contain any of the rules
  whose ids are in $\mathcal{T}_1(I, e, T)$; hence $H'$ is a hypothesis that is
  not accepted by $F$ at the start of the iteration, but which is accepted by
  $F$ at the end of the iteration.
}

\appendixTheorem{cdpi_to_nc1}{
  Let $e$ be a CDPI in $E^{+}$ and $H\subseteq S_{M}$ be a hypothesis that does
  not cover $e$. Let $F$ be the coverage formula returned by
  $\textit{CDPI2NC}(T, H, e)$.
  \begin{enumerate}
    \item $F$ does not accept $H$.
    \item The pair $\langle e, F\rangle$ is a coverage constraint.
  \end{enumerate}
}{
  \proofindent{
    \begin{enumerate}
      \item To prove this part, it suffices to show that $H$ cannot accept the
        disjunct that is added in an arbitrary iteration of either while loop.
        For the first while loop, this holds by definition. For the second,
        this holds because the new disjunct is a conjunction $\lnot
        R^{1}_{id}\land\ldots\land \lnot R^{n}_{id}$ where at least one $R^{i}$
        is in $H$ (if this were not the case then $I$ would be a model of $H$,
        which it cannot be because the first while loop terminated).
      \item When $F$ is returned, the condition of the second while loop must
        be false; hence, there is no $I$ for which $\exists H' \subseteq S_M$
        s.t. $H'$ is not accepted by $F$ and $I\in AAS(e, B\cup H')$.
        Therefore, there is no hypothesis that is not accepted by $F$ that
        covers $e$ -- this is the definition of $\langle e, F\rangle$ being a
        coverage constraint.
    \end{enumerate}
  }
}


==> conflict_analysis/ilasp4_cdpi_positive_extended.tex <==
The approaches for computing coverage constraints from a positive CDPI $e$ in
ILASP3 and ILASP4 can be viewed as two extremes; one computes a complete
translation of $e$, and the other computes a very specific reason why the
current hypothesis does not cover $e$. The first approach, taken by ILASP3, is
likely to lead to very long conflict analysis (and constraint propagation)
times in each iteration, but very few iterations of the CDILP algorithm (as no
example will ever be a counterexample twice). The second approach, taken by
ILASP4, is likely to lead to shorter conflict analysis (and constraint
propagation) times, but may also lead to more iterations of the CDILP algorithm
because the same counterexample could be found many times. The CDPI2NC
algorithm can be tweaked so that it produces a slightly larger constraint,
providing a middle ground between the two approaches.


The basic idea of the alternative CDPI2NCb algorithm is that rather than
selecting just one conjunct from $\mathcal{T}_2(I, e, T)$, it uses the entire
conjunction. Note that this formula is often significantly simpler than the
formula generated by the translation approach of ILASP3.  Our evaluation (in
the next section) shows that ILASP4 with the CDPI2NCb approach to conflict
analysis often outperforms both ILASP3 and ILASP4 with the CDPI2NC approach.
For the rest of the paper, to distinguish between the two approaches, we refer
to ILASP4a and ILASP4b to mean ILASP4 with CDPI2NC and CDPI2NCb, respectively.
The CDPI2NCb algorithm is identical to the CDPI2NC algorithm, other than the
first while loop.

\begin{algorithm}
  \small
  \begin{algorithmic}[1]
    \Procedure{CDPI2NCb}{$T, H, e$}
      \State{$F = \bot$;}
      \While{$\exists I\!\in\! M(H)$, $\exists H'\!\subseteq\!S_M$ s.t.\ $F$ does not accept $H'$ and $I\!\in\!AAS(e, B\cup H')$}
        \State{Fix an arbitrary such $I$;}
        \State{$F = F \lor \mathcal{T}_2(I, e, T)$;}
      \EndWhile
      \While{$\exists I$, $\exists H' \subseteq S_M$ s.t.\ $F$ does not accept $H'$ and $I\in AAS(e, B\cup H')$}
        \State{Fix an arbitrary such $I$;}
        \State{$F = F \lor \mathcal{T}_1(I, e, T)$;}
      \EndWhile
      \State{\textbf{return}\,$F$;}
    \EndProcedure
  \end{algorithmic}
  \caption{$\textit{CDPI2NCb}(T, e)$\label{alg:CDPI2NCb}}
\end{algorithm}

The following two theorems show that CDPI2NCb is guaranteed to complete and is
a valid method for conflict analysis on positive CDPIs.

\appendixTheorem{cdpi_to_nc2_terminate}{
  Let $e$ be a CDPI in $E^{+}$ and $H\subseteq S_{M}$ be a hypothesis that does
  not cover $e$. The procedure $\textit{CDPI2NCb}(T, H, e)$ is guaranteed to
  terminate.
}{
(Similar to the proof of Theorem~\ref{thm:cdpi_to_nc1_terminate}).

  As $F$ is a disjunction, and each iteration of both while loops adds an extra
  disjunct, the hypotheses $H\subseteq S_M$ accepted must either increase or
  stay the same with each iteration (of either while loop). Hence as there are
  a finite number of hypotheses (because $S_M$ is finite), it remains to show
  that for both while loops each iteration adds at least one hypothesis that is
  accepted by $F$ at the end of the iteration that was not accepted by $F$ at
  the start of the iteration.

  In any iteration of the first while loop there is at least one $H' \subseteq
  S_M$ st $H'$ is not accepted by $F$ and $I\in AAS(e, B\cup H')$ (where $I$ is
  the arbitrarily chosen $I$). It therefore suffices to show that $H'$ is
  accepted by the new disjunct $\mathcal{T}_2(I, e, T)$, which is conjunction
  of disjunctions; hence, we must show that $H'$ is accepted by each of these
  disjunctions. Each disjunction $d$ is of the form $R^1_{id}\lor\ldots\lor
  R^{n}_{id}$, where $I$ has at least one non-empty unfounded subset \wrt
  $B\cup e_{ctx}\cup (S_{M}\backslash \lbrace R^{1},\ldots, R^{n}\rbrace)$. If
  $H'$ were not accepted by $d$, then $B\cup e_{ctx} \cup H'$ would be a subset
  of $B\cup e_{ctx} \cup (S_{M}\backslash \lbrace R^{1},\ldots, R^{n}\rbrace)$,
  and $I$ would therefore have at least one non-empty unfounded subset \wrt the
  program, contradicting that $I\in AAS(e, B\cup H')$.

  In any iteration of the second while loop, there must be at least one $H'
  \subseteq S_M$ st $H'$ is not accepted by $F$ and $I\in AAS(e, B\cup H')$.
  $I$ cannot be a model of $H$, or the first while loop would not have
  terminated. Hence, $\mathcal{T}_1(I, e, T)$ must be a non-empty conjunction
  $\lnot R^{1}_{id}\land\ldots\land \lnot R^{n}_{id}$ of rules s.t. $I$ is not
  a model of each $R^{i}$ (it must be non-empty because there is at least one
  rule in $H$, and therefore in $S_{M}$, for which $I$ is not a model). As $I$
  is a model of $B\cup e_{ctx}\cup H'$, $H'$ cannot contain any of the rules
  whose ids are in $\mathcal{T}_1(I, e, T)$; hence $H'$ is a hypothesis that is
  not accepted by $F$ at the start of the iteration, but which is accepted by
  $F$ at the end of the iteration.
}

\appendixTheorem{cdpi_to_nc2}{
  Let $e$ be a CDPI in $E^{+}$ and $H\subseteq S_{M}$ be a hypothesis that does
  not cover $e$. Let $F$ be the coverage formula returned by
  $\textit{CDPI2NCb}(T, H, e)$.
  \begin{enumerate}
    \item $F$ does not accept $H$.
    \item The pair $\langle e, F\rangle$ is a coverage constraint.
  \end{enumerate}
}{
  (Similar to the proof of Theorem~\ref{thm:cdpi_to_nc1}).

  \begin{enumerate}
    \item To prove this part, it suffices to show that $H$ cannot accept the
      disjunct that is added in an arbitrary iteration of either while loop.
      For the first while loop, if this were to hold then $I$ would be an
      answer set of $e$ \wrt $B\cup H$, by Theorem~\ref{thm:translateCDPI}
      ($H$ satisfies $\mathcal{T}_1(I, e, T)$, because $I \in M(H)$). This
      cannot be the case as $H$ does not cover $e$. For the second, this holds
      because the new disjunct is a conjunction $\lnot
      R^{1}_{id}\land\ldots\land \lnot R^{n}_{id}$ where at least one $R^{i}$
      is in $H$ (if this were not the case then $I$ would be a model of $H$,
      which it cannot be because the first while loop terminated).
    \item When $F$ is returned, the condition of the second while loop must be
      false; hence, there is no $I$ for which $\exists H' \subseteq S_M$ s.t.
      $H'$ is not accepted by $F$ and $I\in AAS(e, B\cup H')$.  Therefore,
      there is no hypothesis that is not accepted by $F$ that covers $e$ --
      this is the definition of $\langle e, F\rangle$ being a coverage
      constraint.
  \end{enumerate}
}

